VCD: A Video Conferencing Dataset for Video Compression

Commonly used datasets for evaluating video codecs are all very high quality and not representative of video typically used in video conferencing scenarios. We present the Video Conferencing Dataset (VCD) for evaluating video codecs for real-time communication, the first such dataset focused on video conferencing. VCD includes a wide variety of camera qualities and spatial and temporal information. It includes both desktop and mobile scenarios and two types of video background processing. We report the compression efficiency of H.264, H.265, H.266, and AV1 in low-delay settings on VCD and compare it with the non-video conferencing datasets UVC, MLC-JVC, and HEVC. The results show the source quality and the scenarios have a significant effect on the compression efficiency of all the codecs. VCD enables the evaluation and tuning of codecs for this important scenario. The VCD is publicly available as an open-source dataset at https://github.com/microsoft/VCD.

==> boneyard.tex <==
%    babaknaderi $\vert$ ross.cutler $\vert$ nabakumar $\vert$ yahossei $\vert$ heturbel $\vert$ albert.sadovnikov $\vert$ quan.zou @microsoft.com}

%VCD is the first publicly available corpus designed specifically for evaluating video conferencing use cases. The variety of content in VCD captures the spatial and temporal diversity representative of real-world conferencing streams. Releasing VCD publicly enables standardized benchmarking to drive widespread video conferencing optimization in the research community.

%BVI-DVC: A training database for deep video compression


%\begin{figure*}[tb]
%    \begin{subfigure}[c]{0.24\textwidth}
%        \includegraphics[width=1\textwidth]{figs/quality_distribution_s1.jpg}
%        \caption{}
%    \end{subfigure}    
%    \begin{subfigure}[c]{0.24\textwidth}
%        \includegraphics[width=\textwidth]{figs/quality_distribution_s2.jpg}
%        \caption{}
%    \end{subfigure}
%    \begin{subfigure}[c]{0.24\textwidth}
%        \includegraphics[width=\textwidth]{figs/quality_distribution_s3.jpg}
%        \caption{}
%    \end{subfigure}   
%    \begin{subfigure}[c]{0.24\textwidth}
%        \includegraphics[width=\textwidth]{figs/quality_distribution_s4.jpg}
%        \caption{}
%    \end{subfigure}   
%    \caption{Quality distribution of video sequences in VCD dataset measured in ACR subjective test.}
%    %keep all
%    \label{fig:quality_distribution}
%\end{figure*}

%\begin{mdframed}[hidealllines=true,backgroundcolor=blue!20]
%Analysis items
%\begin{itemize}
%    \item P0: BD-Rate vs MOS - this is the main reason VCD is harder
%    \item P1: BD-Rate of UVG, MLC-JCV, HEVC, VCD on H.265, H.266, AV1 relative to H.264
%    \item P1: RD plot of H.26x and AV1 on UVG, MLC-JCV, HEVC, VCD 
%    \item P1: TI vs SI plots
%    \item P1: MOS distribution
%    \item P2: Demographics
%\end{itemize}
%\end{mdframed}

%In conclusion, the increasing popularity of video conferencing in recent times has underscored the need for high-quality video conferencing compression solutions. Existing video datasets, including MCL-JCV, HEVC, and UVC, have limitations in representing true video conferencing scenarios, as they predominantly focus on high-quality mainstream media content. To address this gap, we introduce VCD, an open-source dataset tailored for video conferencing scenarios, offering a more representative evaluation platform for video codecs. VCD is organized into four video scenarios, mirroring common video types encountered in video conferencing. Additionally, we provide insights into the SI-TI distribution and quality distribution for each of the video scenarios within VCD.

%Furthermore, we demonstrated a notable drop in the compression performance of major video codecs, including HEVC, AV1, and VVC, when evaluated on the VCD dataset compared to their performance on existing general datasets. We attribute this decline in performance to a combination of the inherently lower video quality typically associated with webcam-captured videos from consumer devices, and restrictive compression parameters, such as low-delay encoding settings, used in real-time video conferencing.

%Furthermore, the BD-Rate evaluation can be enhanced by taking into account additional video resolutions. In this paper, we assessed the BD-Rates only at the 1080p resolution, which corresponds to the original resolution of the videos in VCD. However, the compression efficiency of most video codecs significantly diminishes at lower resolutions. Therefore, computing the overall BD-Rates by aggregating results across the various resolutions employed in a video conferencing application would offer improved representation.
